Explaining Neural Networks by Decoding Layer Activations

We present a `CLAssifier-DECoder' architecture (\emph{ClaDec}) which facilitates the comprehension of the output of an arbitrary layer in a neural network (NN). It uses a decoder to transform the non-interpretable representation of the given layer to a representation that is more similar to the domain a human is familiar with. In an image recognition problem, one can recognize what information is represented by a layer by contrasting reconstructed images of \emph{ClaDec} with those of a conventional auto-encoder(AE) serving as reference. We also extend \emph{ClaDec} to allow the trade-off between human interpretability and fidelity. We evaluate our approach for image classification using Convolutional NNs. We show that reconstructed visualizations using encodings from a classifier capture more relevant information for classification than conventional AEs. Relevant code is available at \url{https://github.com/JohnTailor/ClaDec}

==> old/RebuttalResponse.tex <==
We thank the reviewers.

Review 3
* The difference between ClaDec and AE reconstructions might not be understandable (eg. Fig 5)
This question is well-justified, since our interpretation process is cognitively demanding. Comparing ClaDec, AE and the input requires practice. A simpler process yields easier to understand, but less fidel explanations: Compare only the input to ClaDec reconstructions. Comparing 2 images is a simple task. It is easy to see what aspects, eg. shape, color or texture in Fig 5 are preserved and, thus, relevant. Please read also 1st reply to Rev. 4


Review 4
* The claim that reconstructed images can be used as explanations is unsupported. How to use these explanations to draw conclusions about the model?
Theoretical motivation (Fig 3) states that reconstruction quality of images depends on whether that information is deducable from layer activations. That is, the layer is an embedding of the input, which might abstract away some information and keep other. Comparing images of ClaDec and the AE shows what information on the input can be reconstructed, ie. is relevant for the classifier. Given that the encoding does not allow to distinguish between two samples differing in at least one attribute (eg. sweater w/o stripes), the decoder can also not decode this attribute (eg. stripes). In this case, the reconstruction is the average of input samples with similar activations to minimize reconstruction loss - these areas might be less precise/blurry (see Fig 6). Blurriness expresses less relevance. If encodings allow to differentiate attributes, the decoder will reconstruct the attributes (well) to minimize loss. To be able to do so, the input must from the training data distribution. If the decoder has not trained with similar images, it will yield reconstructions that are overall non-realistic but with possibly meaningful parts/features. Such explanations are also interesting. For example, say we feed an MNIST classifier the letter "B" and a reconstruction shows a (funny) mix of a 8 and 1. This means features got activated related to 8 and 1. It's fun to play with random inputs for a decoder (of an AE or classifier), samples for linear interpolation between latent representations of two inputs of an AE are also on the web. See Q2 for Rev 5 for adversarial samples.

*  It lacks strict problem formulation and consequent analysis of the method
The introduction contains a research question with formal aspects on what is used to derive explanations and, more informally, the purpose of these explanations. What an explanation constitutes and how it is derived, is formally defined in the method. This is similar to a number of other papers, eg. LIME paper. We shall also formalize the purpose.

* Novelty is limited
We just point out a story: Comparing to an AE reconstruction was not done by Nguyen et al. 2016 (NIPS), although they noticed artefacts in their GAN-based visualizations of single neurons. They could have tried to reconstruct neurons of an AE and see if this also yields artefacts and assess limitations of their GANs. 4 years and 354 citations later this is still not done

* How to determine if this explanation is reliable or if the explanation method has failed?
If explanations differ strongly from the input, this means that either a mis-classification is going on or the input appears very different from any training data. Please read reply to comment 1 of reviewer 4. For robustness analysis, one might perform a sensitivity analysis using perturbations in the input or layer activations


Review 5
* 1)Classifiers use tricks, such as relying on textures. Decoders/GANs might also do so leading to obscurity
Good point. An empirical reply is: Generative models, ie. GANs have been used for multiple years for explanations (Nguyen et al. 2016, NIPS) without issues. So it should work for our decoder, since GANs are more notorious for artefacts. A better reply is, we compare the results of the AE with the input highlighting issues with the decoder, ie. inappropriate architecture

* Parameter alpha has an important role in Fig 7. This might indicate an error of interpretation.
* Q1) What is the optimal value of alpha?
For alpha=0 we only train the decoder based on the classification loss. Since many kinds of inputs that resemble no similarity to real-word objects can minimize this loss (see adversarial samples) reconstructions are likely non-interpretable as in Fig 7. Table 2 can guide the choice of alpha. Best for fidelity is .001, where performance on downstream tasks is best, showing that reconstructions contain most information of the classifier.

* Lack of comparisons with heatmapping methods and standard sanity checks (Adebayo et al)
It might be no surprise that Adebayo et al only compare gradient based techniques that are very similar in implementation and outcomes, ignoring works such as LIME. It is questionable to what extent their checks apply to non-gradient based methods. For example, cascading randomization makes limited sense in our context, since we do not backpropagate. For data randomization  the interpretation of outcomes is different for our method. Assume explanations look alike for a classifier trained with labels permuted and non-permuted. This means that the classifier encodes the same information as a classifier with non-permuted labels. One might even expect this for layers close to the input, since these representations are fairly robust to dataset changes (as shown by transfer learning). That said, the suggestion is very interesting, however, these sanity checks might require further investigation, calling for a follow up of Adeboya et al.
We agree that a comparison adds value. If we did ``yet another heatmap'', it would be a necessity to compare against other heatmaps. In Fig 3 in Suppl. we provide a brief comparison. We refrain to do so in the main paper, since our explanations are conceptually different. We are afraid that it might create more confusion than clarity given limited space.
Heatmaps are easy to produce, so not doing an experiment but comparing might have been less work

* 3) Use of small resolution datasets limits the scope because CNNs have large receptive fields
The receptive field of a neuron varies across layers. We reconstruct from different layers, ie. we use small and large receptive fields. Also, we use the entire layer (not activations of individual neurons), thus, we do not think that receptive fields are of primary concern

* 4) No new problems that affect CNN classifiers are shown
The goal was to explain layer activations of single samples. We did not attempt to uncover new fundamental issues with CNNs

* 5) Explanations are based on intuitions that might be deceiving. We expect to see explanations based on features like overall geometry
The reason why this is not a concern for us (but for many other methods as the reviewer correctly suggests) is that we compare reconstructions from ClaDec to those of an AE and explicitly focus on differences. Please also read the reply to the 1st question of Reviewer 4.

* Q2) Can you explain mistakes due to adversarial attacks?
For an adversarial sample behavior is analogous as for other incorrectly classified samples, but transitions are expected to be non-comprehensible/extreme depending on the class change - eg. it seems plausible that the big white sole of the sandal leads to a sneaker (see Fig 6), but it's hard to imagine how a plausible transformation looks that turns it into a pant.

* Q3) Should the decoder be symmetric to the encoder? Can it be smaller or larger?
The decoder can be chosen freely. It impacts the quality of reconstruction. It can be used to regulate the complexity of explanations. A small decoder yields less details for both ClaDec and the AE. Thus, the two can differ in fewer ways

* Q4) Is the method limited to sequential networks?
No, one might use eg. RNN encoder/decoder

% -- though the AE encodings contain more information on the input  (lower reconstruction loss) providing evidence for the sanity of our method
